How Physics and Background Attributes Impact Video Transformers in Robotic Manipulation: A Case Study on Planar Pushing

As model and dataset sizes continue to scale in robot learning, the need to understand how the composition and properties of a dataset affect model performance becomes increasingly urgent to ensure cost-effective data collection and model performance. In this work, we empirically investigate how physics attributes (color, friction coefficient, shape) and scene background characteristics, such as the complexity and dynamics of interactions with background objects, influence the performance of Video Transformers in predicting planar pushing trajectories. We investigate three primary questions: How do physics attributes and background scene characteristics influence model performance? What kind of changes in attributes are most detrimental to model generalization? What proportion of fine-tuning data is required to adapt models to novel scenarios? To facilitate this research, we present CloudGripper-Push-1K, a large real-world vision-based robot pushing dataset comprising 1278 hours and 460,000 videos of planar pushing interactions with objects with different physics and background attributes. We also propose Video Occlusion Transformer (VOT), a generic modular video-transformer-based trajectory prediction framework which features 3 choices of 2D-spatial encoders as the subject of our case study. The dataset and source code are available at https://cloudgripper.org.

==> introV2.tex <==
The transformer architecture has established itself as a highly effective tool across a diverse array of sequence-to-sequence problems in natural language processing 
 \cite{NIPS2017_3f5ee243,Radford2019LanguageMA,devlin-etal-2019-bert}, computer vision \cite{dosovitskiy2021an,liu2021swin,Arnab_2021_ICCV}, decision making \cite{NEURIPS2021_7f489f64,NEURIPS2022_b2cac94f,pmlr-v162-zheng22c} and robot manipulation \cite{brohan2022rt,rt22023arxiv,pmlr-v205-shridhar23a}. Among them, video transformers \cite{liu2022video,NEURIPS2021_67f7fb87,arnab2021vivit} are widely studied for video-based downstream tasks and their ability to effectively capture the complex spatio-temporal relationships and long-range dependencies in video data makes them particularly intriguing for robot perception and planning, e.g., visually-grounded robot manipulation through imitation learning \cite{pmlr-v155-dasari21a,10161288,wang2023mimicplay}, robotic video prediction \cite{rakhimov2020latent,gupta2023maskvit,nash2023transframer} and goal-conditioned planning with video demonstrations \cite{9712373,zhao2022p3iv,wang2023event}. However, video transformers are computational expensive \cite{khan2022transformers} and their training requires large video datasets \cite{tong2022videomae} that are usually costly to generate on real robots. In the robotic manipulation context, we investigate the impact of physical and background attributes on the performances of video transformers to alleviate the burden of model pre-training and provide guidance for real-world data collection. 

 
%===================================================================
% FIG. 01
%===================================================================
 
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/1_introduction_v4.pdf}
    % \vspace{-2em}
    % sjin: maybe we should cite cloud gripper hardware paper?
    \caption{\small The dataset, collected with our \textit{CloudGripper} platform - a network of 32 cloud-linked robotic arms, containing robot pushing videos under object and self-occlusion generated from the execution of random planar pushing. (a) The dataset offers RGB videos from both top and bottom cameras. (b) An overview of occlusion percentages across \textit{OccluManip} is also provided. (c) An illustration of target objects and background objects. (d) An example of object occlusion and self-occlusion. }
    \label{fig:dataset_introduction}
    \vspace{-1em}
\end{figure}
%=================================================================
To tackle this problem, we introduce \textit{OccluManip}, a real-world video-based robot pushing dataset encompassing various objects (\textit{Ball}, \textit{Cube}, \textit{Foam}, \textit{Icosahedron}) with distinct physics
attributes (color, friction coefficient, shape) and background settings (static, dynamic, background complexity), resulting in 18 sub-datasets. The combined dataset, collected with our \textit{CloudGripper} system \cite{CloudGripper}, includes 1.4 TB, 460,000 trajectories and 1278 hours of consistent pushing under occlusion videos from a dual-camera system: a top camera view incorporating both self and object occlusion and a bottom camera providing occlusion-free data and precise object location labeling as shown in \textit{Figure. }\ref{fig:dataset_introduction} (a). 
% =================================================================
% FIG. 02
% =================================================================
\begin{figure*}[ht!]
\centering
\includegraphics[width=1.0\linewidth]{figures/2_dataset.pdf}
\vspace{-1.5em}
\caption{\small Selected frames and the according discretized trajectories from \textit{OccluManip} dataset of objects under object and self-occlusion. (a) shows the target object (\textit{Ball}); (b) shows the target object (\textit{Foam}) and one background object; (c) shows the target object (\textit{Cube}) and two background objects; (d) shows the target object (\textit{Icosahedron}) and four backgrounds objects.}
\label{fig:2_dataset}
\vspace{-1em}
\end{figure*}
% ================================================================
% \vspace{-0.1em}


We also present Video Occlusion Transformer (\textit{VOT}), a video-transformer-based network with a generic structure of separate vision and temporal encoding, which takes in the top camera videos with occlusions and predicts a discretized planar positions trace traversed by target object, aligning with the bottom camera view. We refer to this output of grids as a possibility map describing the likely planar positions traced out by the object in the presence of different degrees of occlusion from the top camera perspective. To study the generalisability of video transformers, \textit{VOT} is trained from scratch across all tasks available in \textit{OccluManip}, achieving an average prediction accuracy of 96\%. Zero-shot and few-shot learning are conducted for tasks with various physics attributes and background settings.
% The main contributions of this paper are concluded as below: i) We propose a large-scale video dataset \textit{OccluManip} of robot pushing under occlusion which enables the exploration of how physics attributes, background settings and data scale influence the performance of video transformer and other vision-based large models. The dataset also holds promise for understanding general occlusion problems and occlusion-aware networks with single camera input, resolving the current request of alibrated RGB-D \cite{shridhar2023perceiver} or multi-camera setups \cite{shridhar2022cliport}. ii) A general video-transformer model \textit{GeoT} is designed for successfully fulfilling the tasks in the aforementioned dataset and tackling model generalisability problems. iii) A complete series of experiments are conducted to bridge the gap in understanding what and how do different factors influence the performance of video transformers for robotic tasks.
The main contributions of this paper are: 
\begin{itemize}
    \item We propose a large-scale video dataset \textit{OccluManip} with 1278 hours of robot pushing under occlusion which enables the exploration of how physics attributes, background settings and data scale influence the performance of video transformer and other vision-based large models. The dataset is also potentially useful for understanding general occlusion problems and occlusion-aware networks with single camera input, resolving the current request of calibrated RGB-D \cite{shridhar2023perceiver} or multi-camera setups \cite{shridhar2022cliport}.  
    \item A generic video-transformer model \textit{VOT} is designed to predict possibility maps of planar object trajectories discretized into $12\times16$ grids and with various target objects and changing environmental backgrounds.
    \item We train \textit{VOT} utilizing all the 18 sub-datasets from scratch and perform zero-shot evaluation and fine-tuning across different sub-datasets, namely. tasks, to bridge the gap in understanding what and how physics attributes and background information influence the performance of video transformers for robotic manipulation.
\end{itemize}


==> plot_finetune.tex <==
\definecolor{VOT-1}{RGB}{238,99,82}
\definecolor{VOT-2}{RGB}{89, 205, 144}
\definecolor{SWIN}{RGB}{63, 167, 214}
% \definecolor{Ico}{RGB}{250, 192, 94}

\pgfplotsset{compat=newest}

\begin{figure}[!t]
    % \centering
    \hspace{-2em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Ball}
            \begin{tikzpicture}
             \begin{axis}[
                    xlabel={$Size$},
                    ylabel={$PE$},
                    scaled x ticks=false,
                    every axis x label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        yshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    every axis y label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        xshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    xtick={0,1500, 3000},
                    xticklabels={0,1500 , 3000},
                    label style={font=\small}, % Font size for x and y axis labels
                    tick label style={font=\small}, % Font size for tick labels
                    title style={font=\tiny},
                    width=4.5cm,
                    height=3cm
                ]
            \addplot[color=VOT-1,mark=o] coordinates {
                (300,1050.0)
                (600,1024.0)
                (900,957.9)
                (1200,788.1)
                (1500,859.3)
                (1800,724.8)
                (2100,684.6)
                (2400,664.5)
                (2700,651.9)
                (3000,656.6)
            };
            \addplot[color=VOT-2,mark=square] coordinates {
                (300,1484.8)
                (600,1020.0)
                (900,980.2)
                (1200,886.6)
                (1500,806.3)
                (1800,887.4)
                (2100,792.0)
                (2400,785.1)
                (2700,720.7)
                (3000,601.3)
            };
            \addlegendentry{VOT-1}
            \addlegendentry{VOT-2}
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_ball}
        \end{subfigure}
    \end{minipage}%
    \hspace{2 em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Foam}
            \begin{tikzpicture}
             \begin{axis}[
                        xlabel={$Size$},
                        ylabel={$PE$},
                        scaled x ticks=false,
                        every axis x label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            yshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        every axis y label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            xshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        xtick={0,1500, 3000},
                        xticklabels={0,1500 , 3000},
                        label style={font=\small}, % Font size for x and y axis labels
                        tick label style={font=\small}, % Font size for tick labels
                        title style={font=\tiny},
                        width=4.5cm,
                        height=3cm
                ]
             \addplot[color=VOT-1,mark=o] coordinates {
                (300,102.5)
                (600,105.1)
                (900,96.3)
                (1200,95.8)
                (1500,91.5)
                (1800,70.2)
                (2100,80.2)
                (2400,90.3)
                (2700,56.5)
                (3000,77.3)
              };
              \addplot[color=VOT-2,mark=square] coordinates {
                (300,126.5)
                (600,131.0)
                (900,98.8)
                (1200,79.6)
                (1500,89.8)
                (1800,98.5)
                (2100,88.2)
                (2400,90.4)
                (2700,85.2)
                (3000,82.6)
              };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_foam}
        \end{subfigure}
    \end{minipage}
    
    \vspace{-1.8em} % Space between rows
    \hspace{-1.3 em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Cube}
            \begin{tikzpicture}
             \begin{axis}[
                        xlabel={$Size$},
                        ylabel={$PE$},
                        scaled x ticks=false,
                        every axis x label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            yshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        every axis y label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            xshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        xtick={0,1500, 3000},
                        xticklabels={0,1500 , 3000},
                        label style={font=\small}, % Font size for x and y axis labels
                        tick label style={font=\small}, % Font size for tick labels
                        title style={font=\tiny},
                        width=4.5cm,
                        height=3cm
                    ]
             \addplot[color=VOT-1,mark=o] coordinates {
                (300,601.2)
                (600,412.3)
                (900,276.0)
                (1200,346.2)
                (1500,270.8)
                (1800,182.0)
                (2100,220.4)
                (2400,153.8)
                (2700,158.5)
                (3000,134.0)
            };
            \addplot[color=VOT-2,mark=square] coordinates {
                (300,382.3)
                (600,271.7)
                (900,263.7)
                (1200,272.8)
                (1500,171.3)
                (1800,151.1)
                (2100,161.1)
                (2400,150.6)
                (2700,158.5)
                (3000,148.8)
            };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_cube}
        \end{subfigure}
    \end{minipage}
    \hspace{1 em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Icosahedron}
            \begin{tikzpicture}
         \begin{axis}[
                    xlabel={$Size$},
                    ylabel={$PE$},
                    scaled x ticks=false,
                    every axis x label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        yshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    every axis y label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        xshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    xtick={0,1500, 3000},
                    xticklabels={0,1500 , 3000},
                    label style={font=\small}, % Font size for x and y axis labels
                    tick label style={font=\small}, % Font size for tick labels
                    title style={font=\tiny},
                    width=4.5cm,
                    height=3cm
                ]
            \addplot[color=VOT-1,mark=o] coordinates {
                (300,99.0)
                (600,130.1)
                (900,125.0)
                (1200,94.1)
                (1500,104.7)
                (1800,99.7)
                (2100,70.2)
                (2400,74.6)
                (2700,52.4)
                (3000,62.6)
            };
            \addplot[color=VOT-2,mark=o] coordinates {
                (300,128.4)
                (600,125.5)
                (900,111.9)
                (1200,69.8)
                (1500,96.0)
                (1800,85.4)
                (2100,72.8)
                (2400,65.8)
                (2700,61.6)
                (3000,75.7)
            };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_ico}
        \end{subfigure}
    \end{minipage}

    \caption{\small Models are pre-trained for 90 epochs in the \textit{Single} setting and then fine-tuned and evaluated on a \textit{Quadruple} background setting for 10 epochs. The x-axis represents the fine-tuning dataset size.}
    \label{fig5:fine_tune_curve}
    
\end{figure}

\begin{figure}[!t]
    % \centering
    \hspace{-2em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Ball}
            \begin{tikzpicture}
             \begin{axis}[
                    xlabel={$Size$},
                    ylabel={$PE$},
                    scaled x ticks=false,
                    every axis x label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        yshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    every axis y label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        xshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    xtick={0,3500, 7000},
                    xticklabels={0,3500, 7000},
                    label style={font=\small}, % Font size for x and y axis labels
                    tick label style={font=\small}, % Font size for tick labels
                    title style={font=\tiny},
                    width=4.5cm,
                    height=3cm
                ]
            \addplot[color=SWIN,mark=+] coordinates {
                (700,1020.1)
                (1400,1039.1)
                (2100,942.5)
                (2800,1030.9)
                (3500,977.1)
                (4200,936.1)
                (4900,952.7)
                (5600,888.9)
                (6300,823.8)
                (7000,813.3)
            };
            % \addlegendentry{VOT}
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_ball}
        \end{subfigure}
    \end{minipage}%
    \hspace{2 em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Foam}
            \begin{tikzpicture}
             \begin{axis}[
                        xlabel={$Size$},
                        ylabel={$PE$},
                        scaled x ticks=false,
                        every axis x label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            yshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        every axis y label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            xshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        xtick={0,3500, 7000},
                        xticklabels={0,3500, 7000},
                        label style={font=\small}, % Font size for x and y axis labels
                        tick label style={font=\small}, % Font size for tick labels
                        title style={font=\tiny},
                        width=4.5cm,
                        height=3cm
                ]
             \addplot[color=SWIN,mark=+] coordinates {
                (700,237.2)
                (1400,171.6)
                (2100,142.5)
                (2800,144.2)
                (3500,152.1)
                (4200,143.9)
                (4900,124.7)
                (5600,122.6)
                (6300,125.9)
                (7000,127.2)
            };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_foam}
        \end{subfigure}
    \end{minipage}
    
    \vspace{-1.8em} % Space between rows
    \hspace{-1.3 em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Cube}
            \begin{tikzpicture}
             \begin{axis}[
                        xlabel={$Size$},
                        ylabel={$PE$},
                        scaled x ticks=false,
                        every axis x label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            yshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        every axis y label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            xshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        xtick={0,3500, 7000},
                        xticklabels={0, 3500, 7000},
                        label style={font=\small}, % Font size for x and y axis labels
                        tick label style={font=\small}, % Font size for tick labels
                        title style={font=\tiny},
                        width=4.5cm,
                        height=3cm
                    ]
            \addplot[color=SWIN,mark=+] coordinates {
                (700,484.3)
                (1400,388.0)
                (2100,291.7)
                (2800,276.3)
                (3500,287.6)
                (4200,261.2)
                (4900,234.4)
                (5600,231.0)
                (6300,237.0)
                (7000,208.6)
            };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_cube}
        \end{subfigure}
    \end{minipage}
    \hspace{1 em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Icosahedron}
            \begin{tikzpicture}
         \begin{axis}[
                    xlabel={$Size$},
                    ylabel={$PE$},
                    scaled x ticks=false,
                    every axis x label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        yshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    every axis y label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        xshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    xtick={0,3500, 7000},
                    xticklabels={0,3500, 7000},
                    label style={font=\small}, % Font size for x and y axis labels
                    tick label style={font=\small}, % Font size for tick labels
                    title style={font=\tiny},
                    width=4.5cm,
                    height=3cm
                ]
            \addplot[color=SWIN,mark=+] coordinates {
                (700,273.2)
                (1400,230.1)
                (2100,240.7)
                (2800,214.2)
                (3500,190.0)
                (4200,180.2)
                (4900,171.3)
                (5600,169.8)
                (6300,155.1)
                (7000,155.2)
            };
            \addlegendentry{SWIN}
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_ico}
        \end{subfigure}
    \end{minipage}

    \caption{\small Models are pre-trained for 90 epochs in the \textit{Single} setting and then fine-tuned and evaluated on a \textit{Quadruple} background setting for 10 epochs. The x-axis represents the fine-tuning dataset size.}
    \label{fig5:fine_tune_curve}
    
\end{figure}



==> plot_sat.tex <==
\definecolor{Ball}{RGB}{238,99,82}
\definecolor{Foam}{RGB}{89, 205, 144}
\definecolor{Cube}{RGB}{63, 167, 214}
\definecolor{Ico}{RGB}{250, 192, 94}
\pgfplotsset{compat=newest}
\begin{figure}[h]
    % \centering
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Ball}
            \begin{tikzpicture}
             \begin{axis}[
                    xlabel={$Size$},
                    ylabel={$PE$},
                    scaled x ticks=false,
                    every axis x label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        yshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    every axis y label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        xshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    xtick={0,10000, 20000},
                    xticklabels={0,10000 , 20000},
                    label style={font=\small}, % Font size for x and y axis labels
                    tick label style={font=\small}, % Font size for tick labels
                    title style={font=\tiny},
                    width=4.5cm,
                    height=3cm
                ]
            \addplot[color=Ball,mark=*] coordinates {
                (500,915.0)
                (1000,690.5)
                (5000,460.3)
                (10000,405.4)
                (15000,443.753)
                (20000,413.1)
            };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_ball}
        \end{subfigure}
    \end{minipage}%
    \hspace{1 em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Foam}
            \begin{tikzpicture}
             \begin{axis}[
                        xlabel={$Size$},
                        ylabel={$PE$},
                        scaled x ticks=false,
                        every axis x label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            yshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        every axis y label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            xshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        xtick={0,10000, 20000},
                        xticklabels={0,10000 , 20000},
                        label style={font=\small}, % Font size for x and y axis labels
                        tick label style={font=\small}, % Font size for tick labels
                        title style={font=\tiny},
                        width=4.5cm,
                        height=3cm
                ]
             \addplot[color=Foam,mark=o] coordinates {
                (500,351.5)
                (1000,221.8)
                (5000,103.4)
                (10000,71.9)
                (15000,65.1)
                (20000,61.5)
              };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_foam}
        \end{subfigure}
    \end{minipage}
    
    \vspace{-2em} % Space between rows
    \hspace{0.3em}
    
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Cube}
            \begin{tikzpicture}
             \begin{axis}[
                        xlabel={$Size$},
                        ylabel={$PE$},
                        scaled x ticks=false,
                        every axis x label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            yshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        every axis y label/.style={
                            at={(ticklabel cs:0.5)},
                            anchor=near ticklabel,
                            xshift= 0.5 em % You can adjust this to move the label up or down
                        },
                        xtick={0,10000, 20000},
                        xticklabels={0,10000 , 20000},
                        label style={font=\small}, % Font size for x and y axis labels
                        tick label style={font=\small}, % Font size for tick labels
                        title style={font=\tiny},
                        width=4.5cm,
                        height=3cm
                    ]
             \addplot[color=Cube,mark=square] coordinates {
                (500,45.4)
                (1000,33.2)
                (5000,28.1)
                (10000,17.4)
                (15000,17.6)
                (20000,15.3)
            };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_cube}
        \end{subfigure}
    \end{minipage}
    \hspace{1 em}
    \begin{minipage}{0.2\textwidth}
        \begin{subfigure}[b]{\textwidth}
            \centering
            \caption{Icosahedron}
            \begin{tikzpicture}
         \begin{axis}[
                    xlabel={$Size$},
                    ylabel={$PE$},
                    scaled x ticks=false,
                    every axis x label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        yshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    every axis y label/.style={
                        at={(ticklabel cs:0.5)},
                        anchor=near ticklabel,
                        xshift= 0.5 em % You can adjust this to move the label up or down
                    },
                    xtick={0,10000, 20000},
                    xticklabels={0,10000 , 20000},
                    label style={font=\small}, % Font size for x and y axis labels
                    tick label style={font=\small}, % Font size for tick labels
                    title style={font=\tiny},
                    width=4.5cm,
                    height=3cm
                ]
            \addplot[color=Ico,mark=+] coordinates {
                (500,56.6)
                (1000,58.3)
                (5000,38.3)
                (10000,36.8)
                (15000,37.7)
                (20000,32.9)
            };
            \end{axis}
            \end{tikzpicture}
            \label{subfig:sat_ico}
        \end{subfigure}
    \end{minipage}
    \vspace{-2em}
    \caption{\small Saturation Curve of different target objects in \textit{Single} background setting. The x-axis displays the size of dataset for training. }
    \label{fig4:saturation_curve}
\end{figure}
